DeFi Protocols for Loanable Funds: Interest Rates, Liquidity and Market Efficiency

We coin the term *Protocols for Loanable Funds (PLFs)* to refer to protocols which establish distributed ledger-based markets for loanable funds. PLFs are emerging as one of the main applications within Decentralized Finance (DeFi), and use smart contract code to facilitate the intermediation of loanable funds. In doing so, these protocols allow agents to borrow and save programmatically. Within these protocols, interest rate mechanisms seek to equilibrate the supply and demand for funds. In this paper, we review the methodologies used to set interest rates on three prominent DeFi PLFs, namely Compound, Aave and dYdX. We provide an empirical examination of how these interest rate rules have behaved since their inception in response to differing degrees of liquidity. We then investigate the market efficiency and inter-connectedness between multiple protocols, examining first whether Uncovered Interest Parity holds within a particular protocol and second whether the interest rates for a particular token market show dependence across protocols, developing a Vector Error Correction Model for the dynamics.

==> content/discussion.tex <==
\section{Discussion}
\label{sec:discussion}

\paragraph{Avenues for improvement}

\begin{itemize}
    \item Clustering happens at the kinks, which are close to 100\% utilization --> means that cluster likely near collapse point. 
    \item to the extent that kink clustering occurs, might be better to choose a lower kink point
    \item alternatively, might be better not to use kinks - smooth functions
\end{itemize}

%Current state not ideal, here are some potential improvements. Tie a lot of things together. Inefficeint /efficient markets while high utilization.
%--> Efficiency --> contagion potential (ties the two sections together)

==> stata_outputs/stata_results_dai_original.tex <==
{
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\begin{tabular}{l*{1}{c}}
\toprule
                    &\multicolumn{1}{c}{(1)}\\
                    &\multicolumn{1}{c}{} \\
\midrule
D\_c\_dai             &                     \\
L.\_ce1              &     -0.0695         \\
                    &     (-1.20)         \\
\addlinespace
L.\_ce2              &       0.143         \\
                    &      (1.60)         \\
\addlinespace
LD.Compound DAI     &      -0.216         \\
                    &     (-1.93)         \\
\addlinespace
L2D.Compound DAI    &      -0.186         \\
                    &     (-1.76)         \\
\addlinespace
L3D.Compound DAI    &      -0.413\sym{***}\\
                    &     (-3.98)         \\
\addlinespace
L4D.Compound DAI    &      0.0857         \\
                    &      (0.81)         \\
\addlinespace
LD.Aave DAI         &      -0.165         \\
                    &     (-1.84)         \\
\addlinespace
L2D.Aave DAI        &      -0.115         \\
                    &     (-1.39)         \\
\addlinespace
L3D.Aave DAI        &      -0.119         \\
                    &     (-1.60)         \\
\addlinespace
L4D.Aave DAI        &     -0.0302         \\
                    &     (-0.44)         \\
\addlinespace
LD.dYdX DAI         &      0.0457         \\
                    &      (0.60)         \\
\addlinespace
L2D.dYdX DAI        &     -0.0597         \\
                    &     (-0.86)         \\
\addlinespace
L3D.dYdX DAI        &     -0.0800         \\
                    &     (-1.21)         \\
\addlinespace
L4D.dYdX DAI        &     -0.0182         \\
                    &     (-0.29)         \\
\addlinespace
Constant            &    -0.00102         \\
                    &     (-0.63)         \\
\midrule
D\_a\_dai             &                     \\
L.\_ce1              &       0.381\sym{***}\\
                    &      (4.66)         \\
\addlinespace
L.\_ce2              &      -0.533\sym{***}\\
                    &     (-4.23)         \\
\addlinespace
LD.Compound DAI     &      -0.445\sym{**} \\
                    &     (-2.83)         \\
\addlinespace
L2D.Compound DAI    &     -0.0526         \\
                    &     (-0.35)         \\
\addlinespace
L3D.Compound DAI    &     -0.0603         \\
                    &     (-0.41)         \\
\addlinespace
L4D.Compound DAI    &      -0.495\sym{***}\\
                    &     (-3.32)         \\
\addlinespace
LD.Aave DAI         &       0.171         \\
                    &      (1.35)         \\
\addlinespace
L2D.Aave DAI        &      0.0765         \\
                    &      (0.65)         \\
\addlinespace
L3D.Aave DAI        &      0.0570         \\
                    &      (0.55)         \\
\addlinespace
L4D.Aave DAI        &     -0.0170         \\
                    &     (-0.18)         \\
\addlinespace
LD.dYdX DAI         &      0.0915         \\
                    &      (0.85)         \\
\addlinespace
L2D.dYdX DAI        &     -0.0659         \\
                    &     (-0.67)         \\
\addlinespace
L3D.dYdX DAI        &      0.0207         \\
                    &      (0.22)         \\
\addlinespace
L4D.dYdX DAI        &      0.0599         \\
                    &      (0.69)         \\
\addlinespace
Constant            &   -0.000282         \\
                    &     (-0.12)         \\
\midrule
D\_d\_dai             &                     \\
L.\_ce1              &       0.284\sym{***}\\
                    &      (4.07)         \\
\addlinespace
L.\_ce2              &     -0.0387         \\
                    &     (-0.36)         \\
\addlinespace
LD.Compound DAI     &      -0.723\sym{***}\\
                    &     (-5.40)         \\
\addlinespace
L2D.Compound DAI    &      -0.146         \\
                    &     (-1.15)         \\
\addlinespace
L3D.Compound DAI    &    -0.00323         \\
                    &     (-0.03)         \\
\addlinespace
L4D.Compound DAI    &      -0.788\sym{***}\\
                    &     (-6.21)         \\
\addlinespace
LD.Aave DAI         &      -0.108         \\
                    &     (-1.01)         \\
\addlinespace
L2D.Aave DAI        &       0.192         \\
                    &      (1.92)         \\
\addlinespace
L3D.Aave DAI        &       0.333\sym{***}\\
                    &      (3.74)         \\
\addlinespace
L4D.Aave DAI        &      0.0856         \\
                    &      (1.04)         \\
\addlinespace
LD.dYdX DAI         &      -0.147         \\
                    &     (-1.61)         \\
\addlinespace
L2D.dYdX DAI        &       0.142         \\
                    &      (1.70)         \\
\addlinespace
L3D.dYdX DAI        &      0.0524         \\
                    &      (0.66)         \\
\addlinespace
L4D.dYdX DAI        &     0.00681         \\
                    &      (0.09)         \\
\addlinespace
Constant            &    0.000130         \\
                    &      (0.07)         \\
\midrule
Observations        &         116         \\
\bottomrule
\multicolumn{2}{l}{\footnotesize \textit{t} statistics in parentheses}\\
\multicolumn{2}{l}{\footnotesize \sym{*} \(p<0.05\), \sym{**} \(p<0.01\), \sym{***} \(p<0.001\)}\\
\end{tabular}
}


==> stata_outputs/stata_results_usdc_original.tex <==
{
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\begin{tabular}{l*{1}{c}}
\toprule
                    &\multicolumn{1}{c}{(1)}\\
                    &\multicolumn{1}{c}{} \\
\midrule
D\_c\_usdc            &                     \\
L.\_ce1              &      0.0146         \\
                    &      (0.83)         \\
\addlinespace
L.\_ce2              &      0.0271         \\
                    &      (1.89)         \\
\addlinespace
LD.Compound USDC    &      0.0995         \\
                    &      (1.64)         \\
\addlinespace
L2D.Compound USDC   &     -0.0149         \\
                    &     (-0.25)         \\
\addlinespace
LD.Aave USDC        &     -0.0203         \\
                    &     (-1.60)         \\
\addlinespace
L2D.Aave USDC       &    -0.00742         \\
                    &     (-0.80)         \\
\addlinespace
LD.dYdX USDC        &     -0.0130         \\
                    &     (-0.35)         \\
\addlinespace
L2D.dYdX USDC       &     -0.0332         \\
                    &     (-0.89)         \\
\addlinespace
Constant            &   -0.000189         \\
                    &     (-0.89)         \\
\midrule
D\_a\_usdc            &                     \\
L.\_ce1              &       0.607\sym{***}\\
                    &      (3.42)         \\
\addlinespace
L.\_ce2              &      -0.720\sym{***}\\
                    &     (-4.97)         \\
\addlinespace
LD.Compound USDC    &      -0.397         \\
                    &     (-0.65)         \\
\addlinespace
L2D.Compound USDC   &       0.463         \\
                    &      (0.78)         \\
\addlinespace
LD.Aave USDC        &      -0.164         \\
                    &     (-1.28)         \\
\addlinespace
L2D.Aave USDC       &      0.0425         \\
                    &      (0.45)         \\
\addlinespace
LD.dYdX USDC        &       0.256         \\
                    &      (0.69)         \\
\addlinespace
L2D.dYdX USDC       &      -0.166         \\
                    &     (-0.44)         \\
\addlinespace
Constant            & -0.00000564         \\
                    &     (-0.00)         \\
\midrule
D\_d\_usdc            &                     \\
L.\_ce1              &       0.115\sym{**} \\
                    &      (2.75)         \\
\addlinespace
L.\_ce2              &      0.0200         \\
                    &      (0.59)         \\
\addlinespace
LD.Compound USDC    &      -0.107         \\
                    &     (-0.75)         \\
\addlinespace
L2D.Compound USDC   &       0.172         \\
                    &      (1.23)         \\
\addlinespace
LD.Aave USDC        &    -0.00892         \\
                    &     (-0.30)         \\
\addlinespace
L2D.Aave USDC       &     0.00993         \\
                    &      (0.45)         \\
\addlinespace
LD.dYdX USDC        &       0.154         \\
                    &      (1.76)         \\
\addlinespace
L2D.dYdX USDC       &      0.0349         \\
                    &      (0.39)         \\
\addlinespace
Constant            &   0.0000538         \\
                    &      (0.11)         \\
\midrule
Observations        &         119         \\
\bottomrule
\multicolumn{2}{l}{\footnotesize \textit{t} statistics in parentheses}\\
\multicolumn{2}{l}{\footnotesize \sym{*} \(p<0.05\), \sym{**} \(p<0.01\), \sym{***} \(p<0.001\)}\\
\end{tabular}
}

